Privacy-Preserving Learning of Human Activity Predictors in Smart Environments

The daily activities performed by a disabled or elderly person can be monitored by a smart environment, and the acquired data can be used to learn a predictive model of user behavior. To speed up the learning, several researchers designed collaborative learning systems that use data from multiple users. However, disclosing the daily activities of an elderly or disabled user raises privacy concerns. In this paper, we use state-of-the-art deep neural network-based techniques to learn predictive human activity models in the local, centralized, and federated learning settings. A novel aspect of our work is that we carefully track the temporal evolution of the data available to the learner and the data shared by the user. In contrast to previous work where users shared all their data with the centralized learner, we consider users that aim to preserve their privacy. Thus, they choose between approaches in order to achieve their goals of predictive accuracy while minimizing the shared data. To help users make decisions before disclosing any data, we use machine learning to predict the degree to which a user would benefit from collaborative learning. We validate our approaches on real-world data.

==> NotIncluded.tex <==

% ********************************************
%
%  From the experimental study results
%
% ********************************************


\subsection{Evaluation results on each client data}

We implemented three training approaches to predict daily human activity including local training, centralized training, and federated training. We used Keras library on top of TensorFlow 2.1.0 for implementing local and centralized approaches and TensorFlow-Federated 0.13.1 for implementing federated approach. The detail of each training model is as follows:

\noindent{\bf Local training}
We trained one LSTM network per smart home. Local dataset of the smart home was the only data involved in the training. Each home, started its training on the start day generated by the Poisson random sampling. 
% As we discussed before, each home's dataset was split into a 70\% for training and a 30\% portion of data for evaluation. 
For building the test set, the process was quite the same.
% except that we do not need to separate data based on the day of experiment.
We evaluated the trained model on the test set after each day of training and saved the results. The test set is always 30\% unseen data of each home dataset.
The architecture of the LSTM model was the same for each home. We trained LSTMs with a batch size of 64 and for 500 epochs with early stopping with patience 50 and minimum delta of 0.01. Early stopping is a way to avoid overfitting. This means that after 50 epochs, if the accuracy on validation set (0.2 of train data) changes less than the minimum delta, the model stops further training.

\noindent{\bf Centralized training}
We trained one LSTM model for the centralized dataset in each day of training. The centralized dataset was a concatenation of all available datasets form each of participating home which was also shuffled before training. We used the batch size of 64 for training and applied early stopping similar to the local training. After training, we tested this model on the test set of each home which is 30\% of their all data.

\noindent{\bf Federated training}
% [batch_size, sequence_length, input_dimensionality], 
% We use Adam optimizer~\cite{kingma2014adam}.
% talk about tensorflow and how we implemented the models.
Similar to centralized training, we had only one LSTM with the same architecture.  
 After creating the list of batches of data for each participating home, we gave it to a federated averaging process trainer and initialized it with random weights. 
 The federated averaging process runs training for a fixed number of epochs on each participating home data in parallel. The number of epochs is 1 in this part of our experiments. After training on each data, it averages the updated parameters at the central server. The whole of this training and averaging process is a complete one round of federated training. 
%  This trainer runs each round of training on the items in the list of federated train data in parallel. 
 We ran 20 rounds of training in each training day.
After training, we evaluated this model on the test set of each home which is 30\% of their all data.

Table~\ref{tab:hyperparameters} shows the hyperparameters that we used for each approach. Fig.~\ref{fig:evaluation} shows the result of local, centralized and federated training on test set of a set of different homes.




% \subsubsection{LSTM with a prediction window}



% \begin{table}[]
%     \caption{Categorical accuracy (top) and accuracy with a window of size 3 activities (bottom) on test data for 6 clients in day 60 with local, centralized, and federated approaches.}
%     \centering
%     \begin{tabular}{|>{\centering\arraybackslash}p{2.2cm}|>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.1cm}|>{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}p{1.1cm}|}
    
%     \hline
%       \bf Approach & \bf H1 & \bf H3 & \bf H9 & \bf H17 & \bf H25 & \bf H29 \\
%         \hline
        
%         \end{tabular}
%     \begin{tabular}
%       \vspace{0.05cm}
%   \textbf{Categorical accuracy}
%     \vspace{0.1cm}
%         Local & & & & & & \\
        
%         Centralized & & & & & & \\
        
%         Federated & & & & & & \\
        
%     \end{tabular}
    
%       \vspace{0.05cm}
%   \textbf{accuracy with a window of size 3 activities}
%     \vspace{0.1cm}
    
%     \begin{tabular}{c|c|c|c|c|c|c|}
%         Local & & & & & & \\
        
%         Centralized & & & & & & \\
        
%         Federated & & & & & & \\
        
%     \end{tabular}

%     \label{tab:acc_window}
% \end{table}



% ********************************************
%
%  From the experimental study intro
%
% ********************************************



%\subsection{Datasets preprocessing}
%For the experiments, we use CASAS datasets~\footnote{\href{https://archive.ics.uci.edu/ml/datasets/Human+Activity+Recognition+from+Continuous+Ambient+Sensor+Data}{https://archive.ics.uci.edu/ml/datasets/\\Human+Activity+Recognition+from+Continuous+Ambient+Sensor+Data}}, which are  sets of continuous ambient sensor data for human activity recognition~\cite{cook2010learning}. CASAS includes 30 different datasets collected in homes with volunteer residents while they were performing their daily routines. The datasets have a great diversity. Some of the residents were younger adults, some were healthy older adults, some were older adults with dementia, and some were having pets.


%We chose 3 columns from the attributes in each dataset which are hour of the day, day of the week, and the activity. 
% The task which we are interested is taking a 24 sequence of these features and predict the next activity. 
%\noindent{\bf Activities mapping}
%The activities column in the whole 30 datasets consist of 47 different labels: \textit{step out, toilet, watch TV, leave home, enter home, exercise, sleep out of bed, wake up, read, nap, laundry, bathe, phone, relax, drink,  groom, entertain guests, go to sleep, bed toilet transition, work, work at table, work on computer, work at desk, dress, r2.dress, take medicine, morning meds, evening meds, personal hygiene', r2.personal hygiene', cook, cook breakfast,  r1.cook breakfast, cook lunch, cook dinner, eat, eat breakfast, r2.eat breakfast, eat lunch, eat dinner, wash dishes, wash breakfast dishes', wash lunch dishes, wash dinner dishes, sleep, r1.sleep, other activity.} We grouped these activities into 10 different categories. See 


%\noindent{\bf Downsampling data points with repeated activities to a single data point} We observed that our datasets had different sampling rate from every few seconds to every few minutes or even every few hours. Sampling very frequently results in many sequential data points with the same activity values. For example, when the person is cooking, he or she most probably is still cooking after a few seconds or few minutes. 
% So if the dataset has been collected every few seconds, the same activity appears consecutively. 
% For the sake of simplicity,  We consider the first line of this sequence of repeated activities and remove the next lines with the same activities from the data. The reason is that in a real world scenario, we do not want to make the predictive system rely on sensors reading rates since they might not work the same in every smart home. We want to predict the next activity of the user based on the previous activities alongside hour of the day and day of the week but not the next state of the sensors.


%\noindent{\bf Converting features and outputs to one-hot representation}
%The input of our prediction model is a sequence of three features: hour of the day which is an integer value between 0 and 23, day of the week which is an integer value between 0 (Monday) and 6 (Sunday), and activities that can have 10 different values \{'PERSONAL\_HEALTH\_AND\_HYGIENE', 'EAT', 'DRINK', 'CHORES', 'REST', 'RELAX', 'SOCIAL','WORK', 'LEAVE\_HOME', 'ENTER\_HOME'\}. We encoded the value of each feature to a one-hot representation. One hot encoding converts categorical features to a binary representation. This means that the hour of the week $h_i$ integer value was converted to a list with length 24 of zeros and a one in index $h_i$. Similarly, day of the week integer value $d_i$ was converted to a list with length of 7 and activity string value $a_i$ to a list of zeros and a one. Therefore, the whole size of the input of the predictive model is $24 + 7 + 10 = 41$ and the output size of the model is 10 in which each node corresponds to an activity.

\subsubsection{Local datasets}
% dataset for each home
The function for creating local training and testing gets two input. One input is the home id. For each home id, we select 70\% of each experiment home data for training and 30\% for evaluation. The other input is the day of experiment, $k$, for example. From the the training split (70\% of the data), we separate $k$ days data. Then, we create sequences of training features and a corresponding train label from train data of the first $k$ days.
Each sequence has sequence length of 24 in our experiments since we are more interested to learn long term relationship between the activities during a day.


\subsubsection{Centralized datasets}
% selected datasets concatenated
In order to create centralized training data, first we modeled the arrival time of each smart home by using Poisson random sampling. 
The generated start day for each home were as follows:
$T^{start} = $\{103: 2,
129: 5,
111: 6,
114: 6,
127: 7,
125: 9,
112: 12,
128: 12,
118: 13,
123: 13,
106: 14,
117: 15,
109: 16,
115: 19,
124: 22,
121: 23,
102: 24,
130: 26,
107: 27,
105: 34,
119: 37,
120: 42,
110: 45,
108: 46,
126: 47,
104: 47,
101: 48,
122: 56,
116: 61,
113: 62\}


Similar to local training, first we separate 70\% of the data for training and 30\% for evaluation.
Given a day of training $k$ and the generated start days for each home, we acquired the ids of the available smart homes. Then, we mapped number of days of available data $k - t^{start}_i + 1$ to its corresponding id. In this number of available data, $k$ is the day of training, $t^{start}_i$ is the arrival day of home with id = $i$. 
Having the list of available home ids and their corresponding number of available data, we selected the training data for the day of training $k$ for each available home. After that we concatenated these data together and shuffled them all. 

\subsubsection{Federated datasets}
% the dataset is a list of clients datasets
The procedure for creating training data for federated training was similar to creating training data for centralized training. The train set of each day for participating homes was created from 70\% of data. We create the training sequences and labels. The main difference is that we did not combine data from each home together since each data has to remain at the local place. After creating training data for each home, we shuffled each data separately.
In the federated training setting, it was required to batch the data for each home before training.
Therefore, we batched each created data which means that we sampled data with size of ``batch size'' repeatedly until we processed all the data for that home and we dropped the remainder data  with size of smaller than batch size after this process.
The size of batch size in our experiments was 64. Then appended them to a list so the federated training process can access them separately. The prediction model was trained on these datasets in parallel in each day of training. 


% ********************************************
%
%  from the data generation part
%
% ********************************************

\subsection{Data Generation by Smart Environments}

---- from the intro

In this paper we are considering the problem of learning a predictive model of the user's behavior in smarthomes. We assume that this prediction is done by a smart home component that has access to the recordings of the user.




--- end from the intro


The datasets which we are using have time information, however, It is not realistic to assume that all of the clients start using the system together at day 1. 
Given a set of clients $\{H_{i}\}$ for $i \in \{1, ..., M\}$, we modeled the deployment time of the smart homes as a Poisson process with a mean interarrival rate $\frac{1}{\lambda} = \frac{N}{M}$ in which $\lambda$ is the average arrival rate, $N$ is the arrival interval for all clients, and $M$ is the total number of clients.

We also assume that at day $t$, the data which is accessible to our system is only coming from those clients who have started using the system before $t$.

For example, Fig~\ref{fig:arrival_day} shows a snapshot of what data is available on January 16 for centralized and federated training. 

% In case of local training, each home just uses their own data. In case of centralized training, the system has access to all the data which are in red. In case of federated learning, each client has access to its own red part data. The centralized system has access to updates updates their own model with that, but they send updates to centralized system. We will delve into details of each case in following subsections.

% ******************************************************************
%
%  From earlier versions of the abstract
%
% ******************************************************************


% This model can help the system to better serve user; short or long term divergences from the daily routine, which might need intervention from the smart environment or human caretakers.

%The daily activities performed by a disabled or elderly person can be monitored by a smart environment, and the acquired data can be used to learn a predictive model of user behavior. To speed up the learning, several researchers proposed the use of collaborative learning systems that use data from multiple users. However, disclosing the daily activities of an elderly or disabled user raises privacy concerns. 

%In this paper, we use state-of-the-art deep neural network-based techniques to learn predictive human activity models. In a local learning setting, each user relies on his/her private data to train a model. The centralized learning approach requires the users to disclose their data to a central agent in exchange for a better trained model. In the federated learning approach, the users disclose the parameters of locally trained models. A novel aspect of our work is that we carefully track the data available to the learner at any given time. In this context, we assume that the users choose between approaches in order to achieve their goals of predictive accuracy while maximizing their privacy. To help users make decisions before disclosing any data, we use machine learning to predict the degree to which a user would benefit from collaborative learning. We validate our approaches on real world data. 

%
%In general, it is desirable to minimize the disclosed data.



% ******************************************************************
%
%  From the early version of the intro. Some of these considerations 
%  might be taken into account.
%
% ******************************************************************


--- I am here ---

\BL{Emphasize here that in contrast to many other papers, we are here considering the temporal evolution of the prediction accuracy. Considerations that guide us in one direction at the first day of the participation of the pool, might give us a different advice on day 30. }

We find that indeed, early in the process, the centralized and federated learning approaches outperform local learning. However, this difference decreases in time, and for {\em most} users, after a certain amount of time, the performance of local training overtakes and even exceeds the performance of distributed approaches. 

Clearly, when the local learning model overtakes that of the distributed ones, a rational participant would switch over to local learning, as performance would not justify the privacy loss. This, however, opens up another line of investigation. Even if a local model at some point overtakes the accuracy of the centralized or federated model, by the time of the switchover, the information had already been disclosed. We found that there are a number of homes where the local model overtakes the distributed ones so quickly and decisively that no participation in the federated model is justified. The question is: can we predict that this is the case? Is there a way through which a decision making system can predict, based on minimal, early information (for instance, from the first days or first two days data) whether the distributed learning model will be helpful or not?

In summary, the main contributions of this paper are as follows:

\begin{itemize}
    \item 
    \item We compare the approaches by Minimal data processing was applied to unify the activity labels into a common ontology, and to stagger the starting times with a Poisson arrival model. 
    \item We find that the federated learning model performs competitively with the centralized training for all the use cases. We find that the local learning starts from a lower accuracy early in the training process, but quickly increases in time, and for most scenarios overtakes the distributed approaches. 
    \item We propose early histogram decision - a technique there a classifier makes a decision of participation in the collaborative learning model based on the first days data.
\end{itemize}


In this paper we take a critical look at the learning of activity prediction models from the dual lens of performance and privacy. We compare the centralized, federated and local learning models. In particular we aim to answer the following questions:

\begin{itemize}
    \item does considering the information from other users benefit the prediction model for a given user?
    \item how do federated versus centralized learnign compare through this model?
    \item does the information from a given user (through data upload for centralized or training gradients in the federated learning) benefit the global model?
    \item How does the accuracy of the prediction evolve in time, and is this evolution predictable?
\end{itemize}

There are two ways this training data can be used. In the case of a {\em centralized training} the a central training location will have access to all the data of the $D_\textit{tg}$ data, and uses supervised learning to train a predictor. The advantage of the model is that it uses a standard supervised training model. The disadvantage of the model is the fact that the users need to disclose their data to the centralized system. 

The {\em federated learning} model similarly takes into consideration the data from the users who have joined the learning pool before. However, in this model, the users do not distribute their data to the centralized authority. Instead, they are using the data to train a model locally, and they are communicating to the central authority model updates (in practice, compressed versions of model updates). 

Federated learning had been proposed as a technique that takes advantage of the information collected at various sites, without an explicit transfer of information. Federated learning, executed correctly, can ensure a significant amount of differential privacy~\cite{differential-privacy}. However, attacks against federated learning models had been demonstrated, for instance by injecting fake learning data in the system. Information can also leak out by the participation of the user in the federated learning pool.


% ******************************************************************
%
%  Sharare's introduction
%
% ******************************************************************


% First paragraph
% Talk about human activity prediction. Why it is important.
Smart homes (SHs) and ambient assisted living systems (AALs) have gain a lot of attraction recently by advancements in communication, networking systems, and Internet of things (IoT) devices. Modeling and predicting human activities from smart homes data can improve the quality of life, comfort and safety of the residents. For example, when a resident is not following his or her daily routines such as not taking medicine, not preparing food or too much sleeping, the system can detect potential health problems based on the history of activities. Also, predicting wake up and arrive home activities is a key component for a smart home to be able to achieve energy efficiency. 

% Talk about the challenges of human activity prediction. such as privacy, bandwidth, storage, give some examples.

% Highly efficient use of network bandwidth, Privacy, Low latency, regulatory and economic benefits.

% Second paragraph
% Why not training for each user separately on their device?


% Third paragraph
% talk about federated learning and again human activity prediction problem statement.


% The remainder of this paper is structured around the following contributions:

Our contributions in this paper can be summarised as follows:

\begin{itemize}
  
    \item We suggest federated learning approach to predicting activities of daily living in order to maintain the privacy and security of the clients users in smart homes.

    
    % \item Talk about the results that we have achieved.
    
\end{itemize}

% Method 

% We aim to simulate a realistic scenario for sampling from the homes to participate in centralized and federated training. 
% The training on smart home datasets is different from training on mobile applications where we have thousands of millions of users. 
% Generally, for training on mobile application datasets, we can use simple random selection of clients. 
% Similarly, in our smart homes scenario, we need to decide which homes are selected to participate in each day of training. 

% One way to do this is to consider a start day for each when the home starts to collecting data. Based on these start days, in each day of training we can simulate how many days of data is available from each participating home in that day.




% The start days of smart home participation in training are different from each other. However, they all start taking part in training in a specific interval of time, for example the first $N$ days of the year 2020. 
% To generate the start time for each smart home participation, we use Poisson random sampling. If the number of all smart home dataset is $M$, the average participation event rate in $N$ days is $\lambda = \frac{M}{N}$.


% \begin{algorithm}[t]
% \label{alg:simulation}
% \caption{Generating start day of participating smart homes in centralized and federated training.}
% \SetKwInOut{Require}{require}
% \Require{Number of days in sampling interval: $N$, number of smart home datasets: $M$, List of smart home ids: $ids$}

% Initialize number of participated smart homes to 0: $C = 0$

% Shuffle the list of smart home ids: $shuffle(ids)$

% Calculate participation event rate: $\lambda = \frac{M}{N}$


% \For{each day($i$) in $N$}
% {
% Generate a single random number with Poisson random sampling which is the number of participating smart homes in day($i$): $S_d = P(\lambda, 1)$ 

%     \For{each j = 0, 1, ..., $S_d$}
%     {
%         \If {$C >= M$}
%         {
%             \textit{break}
%          } 
         
%          Assign day($i$) start day to smart home in index $C$ in list of shuffled $ids$
         
%          $C = C + 1$
%     }
% }
% \end{algorithm}


% experiments




% "Local"  - the training data was 70\% of the data from the user itself. We split the training data into sequences of 24. We randomly choose 70\% of the sequences for training and the rest for validation. No other user's data is involved. 30\% for evaluation.



% "Not local" - There are 30 users. We choose 24 users for training. We are splitting their data into  24 sequences. We concatenating all their data. Use the resulting datasets to train an LSTM. We test this LSTM on the remaining 9 users. But for these 9 users, only 30 per cent of the data was used. like in the local case. 

% Federated learning:
% 21 clients participate by providing data for the learning. These are the same training clients as before. You evaluate on the 9 test clients - these are clients that did not provide data for the federated learning. 

% {\footnotesize
% \begin{verbatim}
% --- work
%       --- work at table
%       --- work on computer
%       --- work at desk
% --- relax
%       --- watch TV
%       --- read
% --- SOCIAL_ 
%       --- phone
%       --- entertain guests
% --- REST
%       --- nap
%       --- sleep
%       --- r1.sleep
%       --- sleep out of bed
%       --- go to sleep / wake up <--- the interval between these two are sleep
% --- CHORES
%       --- cook
%           --- r1.cook breakfast
%           --- cook lunch
%           --- cook dinner
%           --- cook
%           --- cook breakfast,
%       --- wash dishes
%           --- wash breakfast dishes
%           --- wash lunch dishes,
%           --- wash dinner dishes
%       --- laundry
% --- FOOD
%       --- eat
%           --- eat breakfast
%           --- r2.eat breakfast
%           --- eat lunch
%           --- eat dinner
% --- PERSONAL_HEALTH_AND_HYGIENE
%       --- HEALTH
%           --- evening meds
%           --- morning meds
%           --- take medicine
%       --- exercise
%       --- toilet
%       --- GROOMING
%           --- groom
%           --- dress
%           --- r2.dress
%       --- PERSONAL_HYGIENE
%           --- bathe
%           --- personal hygiene
%           --- r2.personal hygiene
%       --- exercise
% --- NOT_TRACKED
%     --- other activity
%     --- step out
%     --- leave home / enter home (the interval between)

% Not clear where to put: drink (what this means??? ),  bed toilet transition (is it between sleep and toilet)
% \end{verbatim}
% }


